Evaluating GPT-3 Generated Explanations for Hateful Content Moderation

Recent research has focused on using large language models (LLMs) to generate explanations for hate speech through fine-tuning or prompting. Despite the growing interest in this area, these generated explanations' effectiveness and potential limitations remain poorly understood. A key concern is that these explanations, generated by LLMs, may lead to erroneous judgments about the nature of flagged content by both users and content moderators. For instance, an LLM-generated explanation might inaccurately convince a content moderator that a benign piece of content is hateful. In light of this, we propose an analytical framework for examining hate speech explanations and conducted an extensive survey on evaluating such explanations. Specifically, we prompted GPT-3 to generate explanations for both hateful and non-hateful content, and a survey was conducted with 2,400 unique respondents to evaluate the generated explanations. Our findings reveal that (1) human evaluators rated the GPT-generated explanations as high quality in terms of linguistic fluency, informativeness, persuasiveness, and logical soundness, (2) the persuasive nature of these explanations, however, varied depending on the prompting strategy employed, and (3) this persuasiveness may result in incorrect judgments about the hatefulness of the content. Our study underscores the need for caution in applying LLM-generated explanations for content moderation. Code and results are available at https://github.com/Social-AI-Studio/GPT3-HateEval.

==> ethics.tex <==
\textbf{Data Collection.} We collected publicly available data and removed all personal information (phone, email, postcode, location, and any other privacy information). Any potentially sensitive dialogues were completely removed from our data. No treatment recommendations or diagnostic claims were given in this study. This research is approved and monitored by the University’s Institutional Review Board and performed in accordance with the principle of GDPR (General Data Protection Regulation2) as follows: data processing shall be lawful if it is necessary for the performance of a task carried out in the public interest. Additionally, this study is explored not for any commercial use while merely for scientific purpose and public interest, which are safeguarded by the Art. 89 GDPR. 

\textbf{Annotator Compensation.} We resorted to the Amazon Mechanical Turk crowdsourcing platform to evaluate three artificial indicators (i.e., Empathy, Relevance, and Fluency). The crowdworkers were assessed with 20 random sentences, which averagely took 5-6 minutes to accomplish, and compensated with \$0.8 per HIT (Human Intelligence Task). The compensation was determined based on the US minimum wage of \$7.12 per hour. 

\textbf{Potential Misuse.} Our model is less likely to contribute to depression of users or generate non-empathic expressions (e.g., discrimination, criticism, and antagonism), since the model is based on the assumption that everyone has varying degrees of sensibility and empathy. Additionally, this model removes any sensitive information of users, and it is basically impossible to infer their personalities, preferences, interests, or other private information from the generated dialogues.



==> limitations.tex <==
Our research is limited to the Hatexplain dataset, which focuses on hate speech on Twitter. While our findings give useful insights into the quality and efficacy of GPT-3-generated explanations, they are limited by the dataset's narrow domain. Furthermore, like many other datasets in the field of hate speech detection, the Hatexplain dataset is prone to the intrinsic subjectivity of hate speech annotation. The ground truth of hate speech may vary among annotators, leading to possibly erroneous annotations in some cases. Prior research has pointed to the difficulty of establishing consistent annotation criteria for hate speech and the potential impact on model performance. Moreover, our study is limited by the small sample size of 100 tweets. While we believe this is a sufficient sample to demonstrate our main findings, a larger sample size would increase the statistical power of our results and provide a more comprehensive understanding of the effectiveness of different prompting strategies.

Additionally, we utilized non-expert human annotators to evaluate the GPT-3 model's explanations. While we made steps to assure the correctness of their evaluations, it is probable that some anomalies in their annotations existed. To acquire higher-quality annotations, future research may explore hiring experienced human annotators. Furthermore, our study only looked at the GPT-3 model, so more research is needed to see if comparable results can be found in other LLMs.
